Blockchains through ontologies: the case study of the Ethereum ERC721 standard in OASIS (Extended Version)

Blockchains are gaining momentum due to the interest of industries and people in \emph{decentralized applications} (Dapps), particularly in those for trading assets through digital certificates secured on blockchain, called tokens. As a consequence, providing a clear unambiguous description of any activities carried out on blockchains has become crucial, and we feel the urgency to achieve that description at least for trading. This paper reports on how to leverage the \emph{Ontology for Agents, Systems, and Integration of Services} ("\ONT{}") as a general means for the semantic representation of smart contracts stored on blockchain as software agents. Special attention is paid to non-fungible tokens (NFTs), whose management through the ERC721 standard is presented as a case study.

==> old.tex <==
Tokens are depicted in Fig. \ref{fig:token}. There are four main types of token: 


\begin{itemize}
    \item non-fungible tokens, represented by instances of the class \textit{EthereumSemiFungibleToken}, the latter containing the class \textit{EthereumTokenERC721} that represents non-fungible tokens compliant with the ERC721 standard protocol;
    \item fungible tokens, represented by instances of the class \textit{EthereumFungibleToken}, the latter containing the class \textit{EthereumTokenERC20} that represents fungible tokens compliant with the ERC20 standard protocol;
    \item semi-fungible tokens, represented by instance of the class \textit{EthereumSemiFungibleToken}, the latter containing the class \textit{EthereumTokenERC1155} that represents semi-fungible tokens compliant with the ERC1155 standard protocol;
    \item custom user-defined tokens not compliant with the ERC standard protocols, represented by instances of the class \textit{EthereumCustomToken}.
\end{itemize} 

\begin{figure}[H]
        \centering
        \includegraphics[scale=0.8]{img/EthereumToken.pdf}
        \caption{Ethereum token representation in \ONT{}}
        \label{fig:token}
\end{figure}

The four mentioned classes are defined as subclass of the class \textit{EthereumToken}. Additionally, tokens that have been definitively destroyed are also instances of the class \textit{BurnedEthereumToken}. 


Tokens carry two types of features~\cite{gangemi2002dolce}, a) perdurant features such as the token ID, that never change and are embedded with the entity representing the token and b) endurant features, that change during the life-span of the token and are associated with an instance of the class \textit{EthereumTokenEndurantFeatures} (subclass of \textit{EndurantFeature}), by means of the object-property \textit{hasEthereumTokenEndurantFeature}. The most notable subclass of \textit{EndurantFeature} is the class \textit{EthereumWalletOwnerEndurantFeature}, which describes the wallet of the  token's owner (by means of the data-properties \textit{isInTheWalletOf}). When the endurant features of a token are modified by the smart contract managing it, they became deprecated and replaced by a new set of features by means of a modification activity. Those new features are introduced by means of a fresh instance of the class \textit{EndurantFeature}. Modification of tokens is allowed only if it involves endurant features and hence perdurant features cannot change. Endurant features may be replaced with other endurant features by introducing an instance of the class \textit{EthereumTokenFeatureModificationActivity} which is connected with:

\begin{itemize}
    \item the changed endurant feature, which is also instance of  the class \textit{DeprecatedEthereumTokenEndurantFeature}, by means of the object-property \textit{hasEthereumTokenFeatureModificationSource};
    \item the new endurant feature, by means of the object-property \textit{hasEthereumTokenFeatureModificationResult}.
\end{itemize}

Moreover, the modified endurant feature is connected with the endurant feature that replaces it by means of the object-property \textit{isEthereumTokenFeature
ModifiedIn}, whereas the token embedding the features is connected with the new endurant feature by means of the object-property \textit{hasEthereumTokenEndurantFeature} as described above.

